Molecular interfacial rheology: Lipid membrane shear viscosity

We develop a method to extract the shear viscosity of a lipid membrane from equilibrium molecular dynamics simulations. The method characterizes the rheology of general interfacial systems embedded in three-dimensional media; we term it molecular interfacial rheology. In our simulations the planar bilayer and surrounding water are confined between solid, parallel walls. Following Onsager's regression hypothesis, membrane and water fluctuations are assumed to relax according to the coupled continuum-mechanical equations governing the confined system---which predict that the membrane transverse velocity autocorrelation function (TVACF) decays exponentially, at a rate set by the membrane and water viscosities. The measured TVACF, however, exhibits damped oscillations followed by a slowly decaying tail. We reconcile these behaviors using the Mori--Zwanzig formalism, and extract the wavevector-dependent membrane viscosity from the time-integral of the TVACF. Results from theory and simulations agree over a decade of wavevectors, and extrapolating to long wavelengths yields shear viscosities ranging from 0.064 to 0.18 pN*us/nm across two representative single-component, fluid-phase bilayers. Our results are corroborated by nonequilibrium simulations where a spatially varying in-plane body force is applied to lipid molecules, thus validating the framework of molecular interfacial rheology.

==> custom-commands.tex <==


% custom colors
\definecolor{myCyan}{rgb}{0.0, 0.47, 0.75}
\colorlet{myBlue}{blue!70!green}
\colorlet{myOrange}{red!60!yellow}
\colorlet{myRed}{orange!40!purple}
\colorlet{myGreen}{green!60!blue}           \colorlet{myPurple}{red!60!blue}
\colorlet{myDarkCyan}{myPurple!15!myCyan}
\definecolor{aOrange}{RGB}{191, 87, 0}

\colorlet{cWater}{myCyan}
\colorlet{cHead}{aOrange!80!red}
\colorlet{cTail}{aOrange!70!yellow}
\colorlet{cLipid}{cHead!50!cTail}
\colorlet{cAll}{myPurple}


% new square root definition
% from https://en.wikibooks.org/wiki/LaTeX/Mathematics#Roots
\def\sqrtl{\mathpalette\DHLhksqrt}
\def\DHLhksqrt#1#2{%
\setbox0=\hbox{$#1\sqrt{#2\,}$}\dimen0=\ht0
\advance\dimen0-0.15\ht0
\setbox2=\hbox{\vrule height\ht0 depth -\dimen0}%
{\box0\lower0.4pt\box2}}


% extend figure references
\newcommand{\figpart}[2]{\hyperref[#1]{\ref*{#1}(#2)}}


% abbreviations
\newcommand{\dopc}{\textsc{dopc}\xspace}
\newcommand{\dppc}{\textsc{dppc}\xspace}
\newcommand{\md}{\textsc{md}\xspace}
\newcommand{\mir}{\textsc{mir}\xspace}
\newcommand{\nemd}{\textsc{nemd}\xspace}
\newcommand{\pbcs}{\textsc{pbc}s\xspace}
\newcommand{\sm}{\textsc{sm}\xspace}
\newcommand{\tvacf}{\textsc{tvacf}\xspace}
\newcommand{\tvacfs}{\textsc{tvacf}s\xspace}


% total and partial derivatives
\newcommand{\dd}[2]{\dfrac{\td \mk {#1}}{\td \mk {#2}}}
\newcommand{\ddt}[2]{\dfrac{\td^2 \mk {#1}}{\td \mk {#2}^2}}
\newcommand{\pp}[2]{\dfrac{\partial \mk {#1}}{\partial \mk {#2}}}
\newcommand{\ppt}[2]{\dfrac{\partial^2 \mk {#1}}{\partial \mk {#2}^2}}
\newcommand{\ppth}[2]{\dfrac{\partial^3 \mk {#1}}{\partial \mk {#2}^3}}
\newcommand{\ppf}[2]{\dfrac{\partial^4 \mk {#1}}{\partial \mk {#2}^4}}


% operators
\newcommand{\bfrac}[2]{{^{#1} \! / \mkn _{#2}}} % in-text fractions
\newcommand{\bmcdot}{\bm{\cdot}}
\newcommand{\bmcolon}{\bm{:}}
\newcommand{\jj}[1]{\left\llbracket \mk #1 \mk \right\rrbracket} % jump quantity
\newcommand{\bmnabla}{\bm{\nabla}}
\newcommand{\bmnablaperp}{\bmnabla_{\!\! \perp}}
\newcommand{\bmnablapara}{\bmnabla_{\!\! \smallparallel}}
\newcommand{\nablapara}{\nabla_{\!\! \smallparallel}}
\newcommand{\pdp}{(\, \bmcdot \,)}
\newcommand{\smallparallel}{{\mkern3mu\vphantom{\perp}\vrule depth 0pt\mkern2mu\vrule depth 0pt\mkern3mu}}


% bending moduli
\newcommand{\kb}{k_\tb}
\newcommand{\kc}{k_\tc}
\newcommand{\kg}{k_\tg}


% speed of sound
\newcommand{\cs}{c^{}_\ts}
\newcommand{\cst}{c^2_\ts}


% thermal energy
\newcommand{\kB}{k^{}_{\text{B}}}
\newcommand{\kBT}{\kB \vartheta}


% basis vectors
\newcommand{\bmea}{\bme^{}_\alpha}
\newcommand{\bmeb}{\bme^{}_\beta}
\newcommand{\bmeg}{\bme^{}_\gamma}
\newcommand{\bmej}{\bme_j}
\newcommand{\bmek}{\bme_k}
\newcommand{\bmex}{\bme_x}
\newcommand{\bmey}{\bme_y}
\newcommand{\bmez}{\bme_z}


% text subscripts
\newcommand{\tb}{{\text{b}}}
\newcommand{\tc}{{\text{c}}}
\newcommand{\td}{{\text{d}}}
\newcommand{\tth}{{\text{h}}}
\newcommand{\tg}{{\text{g}}}
\newcommand{\tm}{{\text{m}}}
\newcommand{\ts}{{\text{s}}}
\newcommand{\tw}{{\text{w}}}

\newcommand{\ttc}{t_\tc}


% general membrane and fluid quantities
\newcommand{\ppm}{p^\pm}
\newcommand{\rhom}{\rho^\tm}
\newcommand{\rhow}{\rho^\tw}
\newcommand{\vdiv}{v^{}_{\alpha, \mk \alpha}}
\newcommand{\vj}{v^{}_j}
\newcommand{\vk}{v^{}_k}
\newcommand{\vp}{v^+}
\newcommand{\vm}{v^-}
\newcommand{\vpm}{v^\pm}


% base membrane and fluid quantities
\newcommand{\Jz}{J_0}
\newcommand{\rhoz}{\rho^{}_0}
\newcommand{\rhomz}{\rhom_0}
\newcommand{\rhowz}{\rhow_0}


% perturbed membrane and fluid quantities
\newcommand{\tilfa}{\tilf_\alpha}
\newcommand{\tilpp}{\tilp^+}
\newcommand{\tilpm}{\tilp^-}
\newcommand{\tilppm}{\tilp^\pm}
\newcommand{\tilrhom}{\tilrho^\tm}
\newcommand{\tilvdiv}{\tilv^{}_{\alpha, \mk \alpha}}
\newcommand{\tilvp}{\tilv^+}
\newcommand{\tilvm}{\tilv^-}
\newcommand{\tilvpm}{\tilv^\pm}
\newcommand{\tilvma}{\tilv_\alpha^\tm}
\newcommand{\tilvmdiv}{\tilv_{\alpha, \mk \alpha}^\tm}
\newcommand{\tilvmx}{\tilv_x^\tm}
\newcommand{\tilvmy}{\tilv_y^\tm}


% NEMD quantities
\newcommand{\bmfext}{\bmf^{\text{ext}}}
\newcommand{\bmFext}{\bmF^{\text{ext}}}
\newcommand{\bmFjext}{\bmFext_j}
\newcommand{\fbar}{\bar{f}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\vbaravg}{\langle \mk \vbar \mk \rangle^{}_{\! \Fbar}}
\newcommand{\xiqbar}{\xi^{\qbar}}

% tilde quantities
\newcommand{\tilf}{\tilde{f}}
\newcommand{\tilh}{\tilde{h}}
\newcommand{\tilp}{\tilde{p}}
\newcommand{\tilrho}{\tilde{\rho}}
\newcommand{\tilv}{\tilde{v}}


% physical domain
\newcommand{\ellpar}{\ell_{\smallparallel}}
\newcommand{\ellperp}{\ell_{\! \perp}}
\newcommand{\ellx}{\ell_x}
\newcommand{\elly}{\ell_y}
\newcommand{\ellz}{\ell_z}


% Fourier-transfomed quantities
\newcommand{\hatpq}{\hatp^{\bmq}}
\newcommand{\hatrq}{\hatr^{\bmq}}
\newcommand{\hatrnq}{\hatr^{-\bmq}}
\newcommand{\hatrqperp}{\hatrq_{\mkn \perp}}
\newcommand{\hatrnqperp}{\hatrnq_{\mkn\mkn \perp}}
\newcommand{\hatrhoq}{\hatrho^{\bmq}}
\newcommand{\hatvq}{\hatv^{\bmq}}
\newcommand{\hatvnq}{\hatv^{-\bmq}}
\newcommand{\hatvqpar}{\hatvq_\smallparallel}
\newcommand{\hatvnqpar}{\hatvnq_\smallparallel}
\newcommand{\dothatvqpar}{\dot{\hatv}^{\bmq}_\smallparallel}
\newcommand{\ddothatvqpar}{\ddot{\hatv}^{\bmq}_\smallparallel}
\newcommand{\hatvqperp}{\hatvq_{\mkn\mkn \perp}}
\newcommand{\hatvnqperp}{\hatvnq_{\mkn\mkn \perp}}
\newcommand{\dothatvqperp}{\dot{\hatv}^{\bmq}_{\mkn\mkn \perp}}
\newcommand{\hatbmvq}{\hatbmv^{\bmq}}

\newcommand{\Cq}{C^{\mk \bmq}}
\newcommand{\Cqh}{\Cq_\tth}
\newcommand{\dotCq}{\dot{C}^{\mk \bmq}}
\newcommand{\hatCqv}{\hat{C}^{\mk \bmq}_v}

\newcommand{\tilC}{\tilde{C}}
\newcommand{\tilCq}{\tilC^{\mk \bmq}}
\newcommand{\tilCqh}{\tilCq_\tth}

\newcommand{\Cqpar}{\Cq_{\mkn \smallparallel}}
\newcommand{\dotCqpar}{\dot{C}^{\mk q}_{\mkn \smallparallel}}
\newcommand{\ddotCqpar}{\ddot{C}^{\mk q}_{\mkn \smallparallel}}
\newcommand{\Cqperp}{\Cq_{\mkn\mkn \perp}}
\newcommand{\dotCqperp}{\dot{C}^{\mk q}_{\mkn\mkn \perp}}

\newcommand{\Gq}{G^{\mk \bmq}}

\newcommand{\gammaq}{\gamma^{q}}
\newcommand{\gammaqfit}{\gammaq_{\text{fit}}}
\newcommand{\gammabarq}{\bar{\gamma}^{q}}
\newcommand{\gammaqa}{\gammaq_{\text{a}}}
\newcommand{\gammaqv}{\gammaq_{\text{v}}}
\newcommand{\gammaqpar}{\gamma^{q}_{\smallparallel}}
\newcommand{\gammaqperp}{\gamma^{q}_{\perp}}

\newcommand{\Iq}{I^{\bmq}}
\newcommand{\Iqinf}{\Iq_\infty}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Ibarq}{\Ibar^q}

\newcommand{\Kq}{K^{q}}
\newcommand{\Kqh}{\Kq_{\mkn \tth}}
\newcommand{\tilK}{\tilde{K}}
\newcommand{\tilKq}{\tilK^{q}}

\newcommand{\xiq}{\xi^{q}}
\newcommand{\xiqpar}{\xiq_{\smallparallel}}
\newcommand{\xiqperp}{\xiq_{\perp}}
\newcommand{\xiqw}{\xiq_{\tw}}

\newcommand{\bmuqpar}{\bmu^{\bmq}_\smallparallel}
\newcommand{\bmuqperp}{\bmu^{\bmq}_{\! \perp}}

\newcommand{\na}{n^{}_\alpha}
\newcommand{\nb}{n^{}_\beta}
\newcommand{\qa}{q^{}_\alpha}
\newcommand{\qb}{q^{}_\beta}
\newcommand{\qg}{q^{}_\gamma}
\newcommand{\expq}{e^{i \mk \bmq \bmcdot \bmx}}


% hat quantities
\newcommand{\hatp}{\hat{p}}
\newcommand{\hatr}{\hat{r}}
\newcommand{\hatrho}{\hat{\rho}}
\newcommand{\hatv}{\hat{v}}
\newcommand{\hatbmv}{\bm{\hatv}}


% bold roman letters
\newcommand{\bma}{\bm{a}}
\newcommand{\bme}{\bm{e}}
\newcommand{\bmf}{\bm{f}}
\newcommand{\bmF}{\bm{F}}
\newcommand{\bmj}{\bm{j}}
\newcommand{\bmn}{\bm{n}}
\newcommand{\bmq}{\bm{q}}
\newcommand{\bmr}{\bm{r}}
\newcommand{\bmx}{\bm{x}}
\newcommand{\bmu}{\bm{u}}
\newcommand{\bmv}{\bm{v}}


% bold greek letters
\newcommand{\bmsigma}{\bm{\sigma}}


% math calligraphy
\newcommand{\mco}{\mathcal{O}}
\newcommand{\mcp}{\mathcal{P}}


% spacing
\newcommand{\mk}{\mkern1mu}
\newcommand{\mkn}{\mkern-1mu}
\newcommand{\qqquad}{\qquad\quad}
\newcommand{\qandq}{\quad\text{and}\quad}
\newcommand{\qqandqq}{\qquad\text{and}\qquad}
\newcommand{\qqqandqqq}{\qqquad\text{and}\qqquad}
\newcommand{\qwhereq}{\quad\text{where}\quad}
\newcommand{\qqwhereqq}{\qquad\text{where}\qquad}
\newcommand{\qqqwhereqqq}{\qqquad\text{where}\qqquad}


% for edits
%\newcommand{\as}[1]{\textcolor{red}{#1}}		% material to edit
%\newcommand{\todo}[1]{\textcolor{magenta}{#1}}		% material to edit




